Performance of Ultra-Wideband Impulse Radio in Presence of Impulsive Interference

We analyze the performance of coherent impulsive-radio (IR) ultra-wideband (UWB) channel in presence of the interference generated by concurrent transmissions of the systems with the same impulsive radio. We derive a novel algorithm, using Monte-Carlo method, to calculate a lower bound on the rate that can be achieved using maximum-likelihood estimator. Using this bound we show that such a channel is very robust to interference, in contrast to the nearest-neighbor detector.

==> arbitrary.tex <==

\subsection {Arbitrary Networks}



\subsubsection{Network Topology}

We model the wireless network as a set of $I$ flows, $L$ links, $O$
nodes and $N$ time-slots. Nodes are arbitrary placed, and
sources-destination pairs are arbitrary chosen.



\subsubsection{MAC Layer}

We assume that a schedule consists of time slots $n=1...N$ of
frequency $\alpha_n$. We normalize these lengths such that
$\sum_{n=1}^{N} \alpha_n = 1$. Let us call $\bp^n$ the vector of
transmission powers assigned to links in slot $n$, and let $\bSNR^n$
be the vector of signal-to-noise ratios at receivers of the links,
induced by $\bp^n$. The rate achievable on link $l$ in slot $n$ is
$\bx^n_l = K \, \bSNR^n_l$.  The vector of average rates on the links
is thus $\bxa = \sum_{n=1}^{N} \alpha_n \bx^n$. Since $\bx^n$ has
dimension $L$ (where $L$ is a number of links), by virtue of
Carath\'eodory theorem, it is enough to consider $N \leq L+1$ time
slots of arbitrary lengths $\balpha$ in order to achieve any point in
the convex closure of points $\bx^n$.

We next describe set $\FF(R)$ of feasible average flow rates under a
given routing matrix $R$. It is the set of $\bbf \in \Reals^I$ such
that there exist a schedule $\balpha$, a set of power allocations
$\bp^n$ and a corresponding set of rate allocations $\bx^n$ for all
$n=1\cdots N$, and average rates $\bxa$, such that the following set
of equalities and inequalities are satisfied for all $n=1\cdots N,
i=1\cdots I, l=1\cdots L, o=1\cdots O$:

%\vskip -12pt
\begin{equation}
\begin{array}{rcl}
    f_i &=& f^{\mbox{nmr}}_i (1-C_r) (1-q)^{\nh_i-1}    \\[4pt]
    \bbf^{\mbox{nmr}} &\leq& R\bxa                      \\[4pt]
    \bxa &=& \sum_{n=1}^{L+1} \alpha_n \bx^n    \\[4pt]
    \bx^n_l &=& K \, \bSNR_l(\bp^n)             \\[4pt]
    \bSNR_l(\bp^n) &=& {\bp^n_l h_{ll} \over N + \sum_{k\neq l} \bp^n_k h_{kl}}  \\[4pt]
    1 &=& \sum_{n=1}^{L+1} \alpha_n  \\[4pt]
    1 &\geq& \sum_{l\,:\,l.\mathrm{src} = o} 1_{\{p^n_l>0\}} + 
             \sum_{l\,:\,l.\mathrm{dst} = o} 1_{\{p^n_l>0\}} \\[4pt]
    \bp^n_l &\leq& \PM_l
\end{array} \label{eq:mod}
\end{equation}
where $l.\mathrm{src} = o$ and $l.\mathrm{dst} = o$ are true if node
$o$ is the source or the destination of link $l$, respectively.



\subsubsection{Performance Evaluation}

The goal of the problem is to find the proportionally fair rate
allocation on the set of feasible rates. This is equivalent to the
following optimization problem:
\begin{equation}
U = \max_{R \in \RR, \bbf \in \FF(R)} \sum_{i=1}^I \log( f_i) \label{eq:opt}
\end{equation}
where $\RR$ is the set of possible routing algorithms. The
optimization problem (\ref{eq:opt}) has as free variables routing
matrix $R$, time slots' frequencies $\alpha_n$, and vectors of
transmission powers assigned to links in slot $n$, $\bp^n$. The values
of these variables that solve (\ref{eq:opt}) define the optimal
routing, scheduling and power control in the given network.



